Parsimonious Online Learning with Kernels via Sparse Projections in Function Space

Despite their attractiveness, popular perception is that techniques for nonparametric function approximation do not scale to streaming data due to an intractable growth in the amount of storage they require. To solve this problem in a memory-affordable way, we propose an online technique based on functional stochastic gradient descent in tandem with supervised sparsification based on greedy function subspace projections. The method, called parsimonious online learning with kernels (POLK), provides a controllable tradeoff? between its solution accuracy and the amount of memory it requires. We derive conditions under which the generated function sequence converges almost surely to the optimal function, and we establish that the memory requirement remains finite. We evaluate POLK for kernel multi-class logistic regression and kernel hinge-loss classification on three canonical data sets: a synthetic Gaussian mixture model, the MNIST hand-written digits, and the Brodatz texture database. On all three tasks, we observe a favorable tradeoff of objective function evaluation, classification performance, and complexity of the nonparametric regressor extracted the proposed method.

==> Convergence_GW.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S  E  C  T  I  O  N  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Convergence Analysis}\label{sec:convergence}
%
We turn to studying the theoretical performance of Algorithm \ref{alg:soldd} developed in Section \ref{sec:algorithm}. In particular, we establish that the method, when a diminishing step-size is chosen, is guaranteed to converge to the optimum of \eqref{eq:kernel_stoch_opt}. We further obtain that when a sufficiently small constant step-size is chosen, the limit infimum of the iterate sequence is within a neighborhood of the optimum. In both cases, the convergence behavior depends on the approximation budget used in the online sparsification procedure detailed in Algorithm \ref{alg:komp}.

We also perform a worst-case analysis of the model order of the instantaneous iterates resulting from Algorithm \ref{alg:soldd}, and show that asymptotically the model order depends on that of the optimal $f^*\in\ccalH$.
%
\subsection{Iterate Convergence}\label{subsec:convergence}
%
Before analyzing the proposed method developed in Section \ref{sec:algorithm}, we define key quantities to simplify the analysis and introduce standard assumptions which are necessary to establish convergence. First, define the regularized stochastic functional gradient as
%
\begin{equation}\label{eq:stoch_reg_grad}
\hat{\nabla}_f\ell(f_{t}(\bbx_t),y_t) =\nabla_f\ell(f_{t}(\bbx_t),y_t)  + \lambda f_t
\end{equation}
%
Further define the projected stochastic functional gradient associated with the update in \eqref{eq:projection_hat} as
%
\begin{equation}\label{eq:proj_grad}
\tilde{\nabla}_f\ell(f_{t}(\bbx_t),y_t) =\Big( f_{t} - \ccalP_{ \ccalH_{\bbD_{t+1}}} \Big[
 f_t 
- {\eta}_t \hat{\nabla}_f\ell(f_{t}(\bbx_t),y_t) \Big]\Big)/\eta_t
\end{equation}
%
such that the Hilbert space update of SOLDD [cf. \eqref{eq:projection_hat}] may be expressed as a stochastic descent using projected functional gradients
%
\begin{equation}\label{eq:iterate_tilde}
f_{t+1} = f_t - \eta_t \tilde{\nabla}_f\ell(f_{t}(\bbx_t),y_t) \; .
\end{equation}
%

The definitions \eqref{eq:proj_grad} - \eqref{eq:stoch_reg_grad} will be used to analyze the convergence behavior of the algorithm. Before doing so, observe that the stochastic functional gradient in \eqref{eq:stoch_reg_grad}, based upon the fact that $(\bbx_t, y_t)$ are independent and identically distributed realizations of the random pair $(\bbx, y)$, is an unbiased estimator of the true functional gradient of the expected risk $L(f)$ in \eqref{eq:kernel_stoch_opt}, i.e.
%
\begin{equation}\label{eq:unbiased}
\mathbb{E}[\hat{\nabla}_f\ell(f_{t}(\bbx_t),y_t) \given \ccalF_t ] =\nabla_f R(f_{t})
\end{equation}
%
for all $t$. Next, we formally state technical conditions on the loss functions, data domain, and stochastic approximation errors that are necessary to establish convergence.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%compact data domain
\begin{assumption}\label{as:first}
The feature space $\ccalX\subset\reals^p$ and target domain $\ccalY\subset\reals$ are compact, and the reproducing kernel map may be bounded as
%
\begin{equation}\label{eq:bounded_kernel}
\sup_{\bbx\in\ccalX} \sqrt{\kappa(\bbx, \bbx )} = X < \infty
\end{equation}
%
\end{assumption}

%loss function boundedness
\begin{assumption}\label{as:2}
The instantaneous loss $\ell: \ccalH \times \ccalX \times \ccalY \rightarrow \reals$ is uniformly $C$-Lipschitz continuous for all $z \in \reals $ for a fixed $y\in\ccalY$
%
%
\begin{equation}\label{eq:lipschitz}
| \ell(z, y) - \ell( z', y ) | \leq C |z - z'|
\end{equation}
%
\end{assumption}
%
%loss convexity and differentiability
%
\begin{assumption}\label{as:3}
The loss function $\ell(f(\bbx), y)$ is convex and differentiable with respect to its first (scalar) argument $f(\bbx)$ on $\reals$ for all $\bbx\in\ccalX$ and $y\in\ccalY$.  
\end{assumption}
%
%
%projected stochastic gradient variance
\begin{assumption}\label{as:last}
Let $\ccalF_t$ denote the sigma algebra which measures the algorithm history for times $u\leq t$, i.e. $\ccalF_t=\{\bbx_u, y_u, u_u\}_{u=1}^t$. The projected functional gradient of the regularized instantaneous risk in \eqref{eq:stoch_reg_grad} has finite conditional second moments for each $t$, that is,
%
\begin{equation}\label{eq:stochastic_grad_var}
\mathbb{E} [ \| \tilde{\nabla}_f\ell(f_{t}(\bbx_t),y_t)\|^2_{\ccalH} \mid \ccalF_t ] \leq \sigma^2
\end{equation}
\end{assumption}
%
Assumption \ref{as:first} holds in most practical settings by the data domain itself, and justifies the bounding of the loss in Assumption \ref{as:2}. Taken together, these conditions permit bounding the optimal function $f^*$ in the Hilbert norm, and imply that the worst-case model order is guaranteed to be finite. Variants of Assumption \ref{as:2} appear in the analysis of stochastic descent methods in the kernelized setting \citep{Pontil05erroranalysis,1715525}. Assumption \ref{as:3} is satisfied for supervised learning problems such as logistic regression, support vector machines with the square-hinge-loss, the square loss, among others. Moreover, it is a standard condition in the analysis of descent methods (see \cite{Boyd2004}). Assumption \ref{as:last} is common in stochastic approximation literature, and ensures that the variance of the stochastic approximation is finite. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P  R  O  P  O  S  I  T  I  O  N   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{prop_bounded}
Let Assumptions \ref{as:first}-\ref{as:last} hold and denote $\{f_t \}$ as the sequence generated by Algorithm \ref{alg:soldd} with $f_0 = 0$. Further denote $f^*$ as the optimum defined by \eqref{eq:kernel_stoch_opt}. Both quantities are bounded by the constant $K:={C X}/{\lambda}$ in Hilbert norm for all $t$ as
%
\begin{equation}\label{eq:prop_bounded}
\| f_t \|_{\ccalH} \leq \frac{C X}{\lambda} \; , \qquad \|f^* \|_{\ccalH} \leq \frac{C X}{\lambda}
\end{equation}
%
\end{proposition}
\begin{myproof} See Appendix \ref{apx_prop_bounded}. \end{myproof}

Next we introduce a proposition which quantifies the error due to our sparse stochastic projection scheme in terms of the ration of the sparse approximation budget and the algorithm step-size.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P  R  O  P  O  S  I  T  I  O  N   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{prop1}
Given independent identical realizations $(\bbx_t, y_t)$ of the random pair $(\bbx, y)$, the difference between the projected stochastic functional gradient and the stochastic functional gradient of the regularized instantaneous risk defined by \eqref{eq:proj_grad} and \eqref{eq:stoch_reg_grad}, respectively, is bounded for all $t$ as
%
\begin{equation}\label{eq:prop1}
 \| \tilde{\nabla}_f\ell(f_{t}(\bbx_t),y_t) - \hat{\nabla}_f\ell(f_{t}(\bbx_t),y_t) \|_{\ccalH} \leq \frac{\eps_t}{\eta_t}
\end{equation}
%
where $\eta_t>0$ denotes the algorithm step-size and $\eps_t>0$ is the approximation budget parameter of Algorithm \ref{alg:komp}.
\end{proposition}
%
\begin{myproof} See Appendix \ref{apx_prop1}. \end{myproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  L  E  M  M  A   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lemma1}
Consider the sequence generated $\{f_t \}$ by Algorithm \ref{alg:soldd} with $f_0 = 0$. Under Assumptions \ref{as:first}-\ref{as:last}, the following expected descent relation holds.
%
\begin{align}\label{eq:lemma1}
\E{\| f_{t+1} - f^* \|_{\ccalH}^2 \given \ccalF_t}
	 &\leq\| f_t - f^* \|_{\ccalH}^2
	 - 2 \eta_t [R(f_t) -R(f^*)]  + 2 \eps_t \| f_t - f^* \|_{\ccalH} 
	+ \eta_t^2 \sigma^2 \; . 
\end{align}
%
\end{lemma}
%
\begin{myproof} See Appendix \ref{apx_lemma1}. \end{myproof}

The expected descent relation in Lemma \ref{lemma1} will be used to establish our main results, specifically, the convergence method under either a diminishing or constant learning rate. We first turn our attention to the case where the learning rate is attenuating.

In the following theorem, we obtain that under a diminishing algorithm step-size scheme (non-summable and square-summable), with the sparse approximation budget selection
%
\begin{equation}\label{eq:dim_stepsize}
\sum_{t=1}^\infty \eta_t = \infty \;, \quad \sum_{t=1}^\infty \eta_t^2 < \infty \;, \quad \eps_t = \eta_t^2 \;, 
\end{equation}
%
the sequence converges exactly to the optimal $f^*$ in stated in \eqref{eq:kernel_stoch_opt}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  T  H  E  O  R  E  M  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{theorem_diminishing}
%
Consider the sequence generated $\{f_t \}$ by Algorithm \ref{alg:soldd} with $f_0 = 0$, and denote $f^*$ as the minimizer of the regularized expected risk stated in \eqref{eq:kernel_stoch_opt}. Let Assumptions \ref{as:first}-\ref{as:last} hold and suppose the step-size rules and approximation budget are diminishing as in \eqref{eq:dim_stepsize} with regularizer such that $\eta_t < 1/\lambda$ for all $t$. Then the objective function error sequence converges to null in infimum almost surely as
%
\begin{equation}\label{eq:liminf_objective_thm}
\liminf_{t\rightarrow \infty} R(f_t) - R(f^*) = 0 \qquad\text{ a.s.}
\end{equation}
%
Moreover, the sequence of functions $\{f_t \}$ converges almost surely to the optimum $f^*$ as
%
\begin{equation}\label{eq:sequence_conv_thm}
\lim_{t\rightarrow \infty} \| f_t - f^*\|_{\ccalH}^2 = 0 \qquad \text{ a.s.}
\end{equation}
%
\end{theorem}
%
\begin{myproof} See Appendix \ref{apx_theorem_diminishing}. \end{myproof}

The result in Theorem \ref{theorem_diminishing} states that when a diminishing algorithm step-size is chosen as, e.g. $\eta_t=\ccalO(1/t)$, and the approximation budget that dictates the size of the sparse stochastic subspaces onto which the iterates are projected is selected as $\eps_t=\eta_t^2$, we obtain exact convergence to the optimizer of the regularized expected risk in \eqref{eq:kernel_stoch_opt}. If instead we consider a constant algorithm step-size $\eta_t=\eta$ and approximation budget $\eps_t=\eps=\ccalO(\eta^{3/2})$, we obtain that the iterates converge to a neighborhood of the optimum, as we state next.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  T  H  E  O  R  E  M  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem}\label{theorem_constant}
Denote $\{f_t \}$ as the sequence generated by Algorithm \ref{alg:soldd} with $f_0 = 0$, and denote $f^*$ as the minimizer of the regularized expected risk stated in \eqref{eq:kernel_stoch_opt}. Let Assumptions \ref{as:first}-\ref{as:last} hold, and given regularizer $\lambda > 0$, suppose a constant algorithm step-size $\eta_t=\eta$ is chosen such that $\eta < 1/\lambda$, and the sparse approximation budget satisfies $\eps=(C \eta)^{3/2}=\ccalO(\eta^{3/2})$, where $C$ is a scaler bounding the instantaneous gradient [cf. \eqref{eq:lipschitz}]. Then the algorithm converges to a neighborhood almost surely as
%
\begin{equation}\label{eq:theorem_constant}
%
\liminf_{t\rightarrow \infty} \|f_t - f^* \|_\ccalH \leq \frac{\sqrt{\eta}}{\lambda}\Big(C^{3/2} +  \sqrt{C^{3} + \lambda  \sigma^2 }\Big) = \ccalO(\sqrt{\eta}) \qquad \text{ a.s. }
%
\end{equation}
%
\end{theorem}
\begin{myproof} See Appendix \ref{apx_theorem_constant}. \end{myproof}
%
\subsection{Model Order Control}\label{subsec:model_order}
%
In this subsection, we establish that the sequence of functions $\{f_t\}$ generated by Algorithm \ref{alg:soldd}, when a constant algorithm step-size is selected, is parameterized by a kernel dictionary which is guaranteed to have finitely many elements, i.e., its the model order remains bounded. We obtain that the worst-case bound on the model order of $f_t$ is depends by the topological properties of the feature space $\ccalX$, the Lipschitz constant of the instantaneous loss, and the radius of convergence $\Delta$ defined in Theorem \ref{theorem_constant}.

\begin{theorem}\label{theorem_model_order}
Denote $f_t$ as the function sequence defined by Algorithm \ref{alg:soldd} with constant step-size $\eta_t=\eta<1/\lambda$ and approximation budget $\eps=(K \eta)^{3/2}$ where $K>0$ is an arbitrary positive scalar. Let $M_t$ be the model order of $f_t$ i.e., the number of columns of the dictionary $\bbD_t$ which parameterizes $f_t$. Then there exists a finite upper bound $M^\infty$ such that, for all $t\geq0$, the model order is always bounded as $M_t\leq M^\infty$.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%    P   R   O   O   F    %%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproof}
We shall proceed by first establishing that, for the purpose of analyzing model order growth, the approximation error associated with removing the most recent feature vector, $\bbx_t$, may be considered in lieu of the termination criterion of Algorithm \ref{alg:komp}.  We then show that this error is a weighted set distance from $k(\bbx_t,\cdot)$ to the Hilbert subspace $\ccalH_{\bbD_t}$ defined by $\bbD_t$.  Finally, by considering the dictionary construction scheme and using the fact that $\ccalX$ is compact, we make a topological argument that the number of dictionary elements is finite.

Begin by considering the termination criterion of Algorithm \ref{alg:komp}, specifically for the very first iteration of the outermost while loop.  Algorithm \ref{alg:komp} will terminate at this iteration if and only if
\begin{equation}\label{eq:komp_no_terminate}
\min_{j=1,\dots,{M_t + 1}} \gamma_j \leq \eps \;
\end{equation}
is satisfied.  If it is, and only if it is, Algorithm \ref{alg:komp} will terminate without having removed any points, and the latest feature point $\bbx_t$ will be added to the model for $f_{t+1}$ and $M_{t+1} > M_t$ (otherwise, at least one point will be removed and $M_{t+1} \leq M_t$).  Given that the error associated with removing $\bbx_t$ is denoted here as $\gamma_{M_t+1}$, note that an increase in model order necessarily implies that $\gamma_{M_t+1} > \epsilon$.  Taking the contrapositive of the previous statement, we have that
\begin{align}
\left[ \gamma_{M_t+1} \leq \epsilon \right] \Rightarrow \left[ M_{t+1} \leq M_t \right] .
\end{align}

We now turn our attention to the quantity $\gamma_{M_t+1}$, which is given by
\begin{align}\label{eq:min_gamma_expand}
\gamma_{M_t+1}
			&=\min_{\bbu\in\reals^{{M_t}}} \Big\|(1-\eta\lambda){f}_t - \eta\ell'({f}_t(\bbx_t),\bby_t)\kappa(\bbx_t,\cdot) -\sum_{k \in \ccalI \setminus \{M_t + 1\}} u_k \kappa(\bbd_k, \cdot) \Big\|_{\ccalH} \\
			&=\min_{\bbu\in\reals^{{M_t}}} \Big\|(1 - \eta \lambda) \!\!\! \!\!\!\sum_{k \in \ccalI \setminus \{M_t + 1\}} \!\!\!  \!\!\!w_k \kappa(\bbd_k, \cdot)- \eta\ell'({f}_t(\bbx_t),\bby_t)\kappa(\bbx_t,\cdot)   -\!\!\! \sum_{k \in \ccalI \setminus \{M_t + 1\}} \!\!\! \!\!\! u_k \kappa(\bbd_k, \cdot)\Big\|_{\ccalH} \; , \nonumber
\end{align}
where we denote the $k^\text{th}$ column of $\bbD_t$ as $\bbd_k$. Considering the square of the expression inside the minimization and expanding terms, we obtain
\begin{align}\label{eq:error_expansion}
\Big\|(1 -& \eta \lambda) \!\!\! \!\!\!\sum_{k \in \ccalI \setminus \{M_t + 1\}} \!\!\!  \!\!\!w_k \kappa(\bbd_k, \cdot)- \eta\ell'({f}_t(\bbx_t),\bby_t)\kappa(\bbx_t,\cdot)   -\!\!\! \sum_{k \in \ccalI \setminus \{M_t + 1\}} \!\!\! \!\!\! u_k \kappa(\bbd_k, \cdot)\Big\|_{\ccalH}^2  \\
&= (1-\eta \lambda)^2 \bbw^T \bbK_{\bbD_t, \bbD_t} \bbw 
+ \eta^2 \ell'({f}_t(\bbx_t),\bby_t)^2\kappa(\bbx_t,\bbx_t)
+ \bbu^T \bbK_{\bbD_t, \bbD_t} \bbu  \nonumber \\
&\quad\!-\! 2(1\!-\!\eta \lambda\!) \eta\ell'\!({f}_t(\bbx_t),\bby_t)^2 \bbw^T\! \bbkappa_{\bbD_t}(\bbx_t) 
\!+\! 2 \eta^2 \ell'({f}_t(\bbx_t),\bby_t)\bbu^T\!\bbkappa_{\bbD_t}(\bbx_t) \!
- \!\!2 (1\!-\!\eta \lambda) \bbw^T\! \bbK_{\bbD_t, \bbD_t} \bbu  . \nonumber
\end{align}
To minimize this expression, we compute the stationary solution of \eqref{eq:error_expansion} with respect to $\bbu \in \reals^{M_t}$ and solve for the minimizing $\tbu^*$.  Using techniques similar to those used in \eqref{eq:proximal_hilbert_representer} - \eqref{eq:hatparam_update}, $\tbu^*$ is given by
\begin{align}\label{eq:minimal_weights}
\tbu^* = (1-\eta \lambda) \bbw - \eta \ell'({f}_t(\bbx_t),\bby_t) \bbK_{\bbD_t, \bbD_t}^{-1} \bbkappa_{\bbD_t}(\bbx_t) \; .
\end{align}
Now, substituting $\tbu^*$ in \eqref{eq:minimal_weights} into \eqref{eq:min_gamma_expand} and using ${f}_{t}(\cdot)=\bbw^T \bbkappa_{\bbD_t}(\cdot)$ and $\sum_k u_k \kappa(\bbd_k, \cdot)= \bbu^T \bbkappa_{\bbD_t}(\cdot)$, the right-hand side of \eqref{eq:min_gamma_expand} can be written as
\begin{align}\label{eq:min_gamma_optimal_weights}
&\Big\| (1-\eta \lambda) \bbw^T\bbkappa_{\bbD_t}(\cdot) - \eta\ell'({f}_t(\bbx_t),\bby_t)\kappa(\bbx_t,\cdot) -  \bbu^T \bbkappa_{\bbD_t}(\cdot) \Big\|_{\ccalH} \\
&\quad =\! \Big\|(1\!-\!\eta\lambda\!)\bbw^T\! \bbkappa_{\bbD_t}(\cdot) \!
 -\! \eta \ell'\!({f}_t(\bbx_t),\bby_t)\kappa(\bbx_t,\!\cdot\!) \!
-\! \! [(1\!-\!\eta\lambda)\bbw \!- \!\eta \ell'\!({f}_t(\bbx_t),\bby_t)\bbK_{\bbD_t, \bbD_t}^{-1} \bbkappa_{\bbD_t}(\bbx_t)]^T 
\!\!\bbkappa_{\bbD_t}(\cdot) \! \Big\|_{\ccalH}  .\nonumber
\end{align}
The above expression may be further simplified by canceling like terms $(1-\eta\lambda)\bbw^T\! \bbkappa_{\bbD_t}(\cdot)$ and moving the common factor $\eta |\ell'({f}_t(\bbx_t),\bby_t) |$ outside the norm, i.e.,
\begin{align}\label{eq:min_gamma_optimal_weights2}
\gamma_{M_t+1} = \eta|\ell'({f}_t(\bbx_t),\bby_t) | \Big\|  \kappa(\bbx_t,\cdot) 
  - [\bbK_{\bbD_t, \bbD_t}^{-1} \bbkappa_{\bbD_t}(\bbx_t)]^T
   \bbkappa_{\bbD_t}(\cdot) \Big\|_{\ccalH} \; . 
\end{align}
The expression on the right-hand side of \eqref{eq:min_gamma_optimal_weights2} may be identified as a function of the set distance between kernel function defined by the newest point, $\phi(\bbx_t ) = \kappa(\bbx_t, \cdot)$, and the Hilbert subspace $\ccalH_{\bbD_t}$ for the fixed dictionary $\bbD_t$. To see this, note that the distance from $\kappa(\bbx_t,\cdot)$ to the subspace $\ccalH_{\bbD_t}$ is defined as
\begin{align}\label{eq:subspace_dist}
\text{dist}( \kappa(\bbx_t, \cdot) , \ccalH_{\bbD_t}) 
= \min_{f\in\ccalH_{\bbD}} \| \kappa(\bbx_t, \cdot) - f(\cdot) \|_{\ccalH} 
= \min_{\bbv\in \reals^{M_t}} \| \kappa(\bbx_t, \cdot) - \bbv^T \bbkappa_{\bbD_t}(\cdot) \|_{\ccalH} \; ,
\end{align}
which, upon substituting the minimizing $\tbv^*=\bbK_{\bbD_t, \bbD_t}^{-1}\bbkappa_{\bbD_t}(\bbx_t)$, is given by
\begin{align}\label{eq:subspace_dist2}
\text{dist}(\kappa(\bbx_t, \cdot) , \ccalH_{\bbD_t}) =  \Big\|  \kappa(\bbx_t,\cdot) 
  - [\bbK_{\bbD_t, \bbD_t}^{-1} \bbkappa_{\bbD_t}(\bbx_t)]^T
   \bbkappa_{\bbD_t}(\cdot) \Big\|_{\ccalH} \; .
\end{align}
Notice now that the right-hand side of \eqref{eq:min_gamma_optimal_weights2} may be identified as the distance to the subspace $\ccalH_{\bbD_t}$ in \eqref{eq:subspace_dist2} scaled by a factor of $\eta|\ell'({f}_t(\bbx_t),\bby_t) | $, i.e.,
%
\begin{align}
\gamma_{M_t+1} = \eta|\ell'({f}_t(\bbx_t),\bby_t)| \text{dist}(\kappa(\bbx_t,\cdot),\ccalH_{\bbD_t}) .
\end{align}
%
Returning to our analysis of model order growth, we have now established the condition $\left[ \eta|\ell'(f_t(\bbx_t),\bby_t)|\text{dist}(\kappa(\bbx_t,\cdot),\ccalH_{\bbD_t}) \leq \epsilon \right] \;\; \Rightarrow \;\; \left[ M_{t+1} \leq M_t\right]$, i.e.,
\begin{align}
\left[\text{dist}(\kappa(\bbx_t,\cdot),\ccalH_{\bbD_t}) \leq \frac{\epsilon}{\eta|\ell'(f_t(\bbx_t),\bby_t)|} \right] \;\;\; \Rightarrow \;\;\; \left[ M_{t+1} \leq M_t \right]
\end{align}
Using the selection $\epsilon=K\eta^{3/2}$, the above can be written as $\left[\text{dist}(\kappa(\bbx_t,\cdot),\ccalH_{\bbD_t}) \leq \frac{K\sqrt{\eta}}{|\ell'(f_t(\bbx_t),\bby_t)|} \right] \;\;\; \Rightarrow \;\;\; \left[ M_{t+1} \leq M_t \right]$, which, due to the $C$-Lipschitz continuity of $\ell$ in Assumption \ref{as:2}, leads to
\begin{align}
\label{eq:min_gamma1}
\left[\text{dist}(\kappa(\bbx_t,\cdot),\ccalH_{\bbD_t}) \leq \frac{K\sqrt{\eta}}{C} \right] \;\;\; \Rightarrow \;\;\; \left[ M_{t+1} \leq M_t \right] \; .
\end{align}
The contrapositive of the above expression tells us that growth in the model order implies that the condition
\begin{align}
\label{eq:min_gamma2}
\left[\text{dist}(\kappa(\bbx_t,\cdot),\ccalH_{\bbD_t}) > \frac{K\sqrt{\eta}}{C} \right]
\end{align}
is true.  Therefore, each time a new point is added to the model, the corresponding kernel function is guaranteed to be at least a distance of $\frac{K\sqrt{\eta}}{C}$ from every other kernel function in the current model, i.e., for distinct dictionary points $\bbd_k$ and $\bbd_j$  for $j,k\in\{1,\dots,M_t\}$, $\|\phi(\bbd_j) - \phi(\bbd_k) \|_2 > \frac{K\sqrt{\eta}}{C}$.  We shall now proceed in a manner similar to the proof of Theorem 3.1 in \cite{1315946}.  Since $\ccalX$ is compact and $\kappa$ is continuous, the range $\phi(\ccalX) $ (where $\phi(\bbx)=\kappa(\bbx,\cdot)$ for $\bbx \in \ccalX$) of the kernel transformation of feature space $\ccalX$ is compact. Therefore, the number of balls of radius $\delta$ (here, $\delta = \frac{K\sqrt{\eta}}{C}$) needed to cover the set $\phi(\ccalX)$ is finite (see, e.g., \cite{anthony2009neural}).  Therefore, for some finite $M^\infty$, if $M_t = M^\infty$, the left-hand side of \eqref{eq:min_gamma1} is guaranteed to be true, and thus $M_{t+1} \leq M^\infty$ for all $t$.
\end{myproof}

==> Simulations.tex <==
%!TEX root = root.tex
\section{Numerical analysis}
\label{sec:simulations}


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%    M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we study the numerical performance of the doubly stochastic approximation algorithms developed in Sections \ref{sec:rapsa}-\ref{sec:asyn} by first considering a linear regression problem. We then use RAPSA to develop a visual classifier to distinguish between distinct hand-written digits. 

\subsection{Linear Regression}\label{subsec:lmmse}

We consider a setting in which observations $\bbz_n\in\reals^q$ are collected which are noisy linear transformations $\bbz_{n}=\bbH_n \bbx + \bbw_{n}$ of a signal $\bbx\in\reals^p$ which we would like to estimate, and $\bbw \sim \ccalN(0, \sigma^2 I_q)$ is a Gaussian random variable. For a finite set of samples $N$, the optimal $\bbx^*$ is computed as the least squares estimate $\bbx^*:=\argmin_{\bbx\in\reals^p } ({1}/{N})\sum_{n=1}^N \|\bbH_{n}\bbx- \bbz_{n}\|^2$. We run RAPSA on LMMSE estimation problem instances where $q=1$, $p=1024$, and $N=10^4$ samples are given. The observation matrices $\bbH_n \in \reals^{q\times p}$, when stacked over all $n$ (an $N \times p$ matrix), are generated from a matrix normal distribution whose mean is a tri-diagonal matrix. The main diagonal is $2$, while the super and sub-diagonals are all set to $-1/2$. Moreover, the true signal has entries chosen uniformly at random from the fractions $\bbx\in \{1,\dots,p\}/p$. Additionally, the noise variance perturbing the observations is set to $\sigma^2=10^{-2}$. We assume that the number of processors $I=16$ is fixed and each processor is in charge of $1$ block. We consider different number of blocks $B=\{16,32,64,128\}$. Note that when the number of blocks is $B$, there are $p/B=1024/B$ coordinates in each block. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}\centering
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$]{
\includegraphics[width=0.48\linewidth,height=0.28\linewidth]
{figures/rapsa_linear_regression_empiricalrisk_constant_iter.eps}\label{subfig:rapsa_linear_constant_a}}
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.48\linewidth,height=0.28\linewidth]
{figures/rapsa_linear_regression_empiricalrisk_constant_features.eps}\label{subfig:rapsa_linear_constant_b}}
%
\caption{RAPSA on a linear regression (quadratic minimization) problem with signal dimension $p=1024$ for $N=10^3$ iterations with mini-batch size $L=10$ for different number of blocks $B=\{16,32,64,128\}$ initialized as $10^4 \times \bbone$. We use constant step-size $\gamma^t= \gamma=10^{-2}$. Convergence is in terms of number of iterations is best when the number of blocks updated per iteration is equal to the number of processors ($B=16$, corresponding to parallelized SGD), but comparable across the different cases in terms of number of features processed. This shows that there is no price payed in terms of convergence speed for reducing the computation complexity per iteration.} \label{fig:rapsa_linear_constant}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%LMMSE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%
%%%   R   A   P   S   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%constant step-size RAPSA
{\bf Results for RAPSA} We first consider the algorithm performance of RAPSA (Algorithm \ref{algo_RAPSA}) when using a constant step-size $\gamma^t=\gamma=10^{-2}$. The size of mini-batch is set as $L=10$ in the subsequent experiments. To determine the advantages of incomplete randomized parallel processing, we vary the number of coordinates updated at each iteration. In the case that $B=16$, $B=32$, $B=64$, and $B=128$, in which case the number of updated coordinates per iteration are $1024$, $512$, $256$, and $128$, respectively. Notice that the case that $B=16$ can be interpreted as parallel SGD, which is mathematically equivalent to Hogwild! \citep{Niu11hogwild:a}, since all the coordinates are updated per iteration, while in other cases $B>16$ only a subset of $1024$ coordinates are updated. 

 Fig. \ref{subfig:rapsa_linear_constant_a} illustrates the convergence path of RAPSA's objective error sequence defined as $F(\bbx^t) - F(\bbx^*)$ with $F(\bbx) = ({1}/{N})\sum_{n=1}^N \|\bbH_{n}\bbx- \bbz_{n}\|^2 $
  as compared with the number of iterations $t$. In terms of iteration $t$, we observe that the algorithm performance is best when the number of processors equals the number of blocks, corresponding to parallelized stochastic gradient method. However, comparing algorithm performance over iteration $t$ across varying numbers of blocks updates is unfair. If RAPSA is run on a problem for which $B=32$, then at iteration $t$ it has only processed {\it half} the data that parallel SGD, i.e., $B=16$, has processed by the same iteration. Thus for completeness we also consider the algorithm performance in terms of number of features processed $\tdp_t$ which is given by $\tdp_t=ptI/B$.
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}\centering
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$]{
\includegraphics[width=0.48\linewidth,height=0.28\linewidth]
{figures/rapsa_linear_regression_empiricalrisk_hybrid_iter.eps}\label{subfig:rapsa_linear_hybrid_a}}
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.48\linewidth,height=0.28\linewidth]
{figures/rapsa_linear_regression_empiricalrisk_hybrid_features.eps}\label{subfig:rapsa_linear_hybrid_b}}
%
\caption{RAPSA on a linear regression problem with signal dimension $p=1024$ for $N=10^3$ iterations with mini-batch size $L=1$0 for different number of blocks $B=\{16,32,64,128\}$ using initialization $\bbx_0 = 10^4 \times \bbone$. We use hybrid step-size $\gamma^t= \min(10^{-1.5},10^{-1.5} \tilde{T}_0/t)$ with annealing rate $\tilde{T}_0=400$. Convergence is faster with smaller $B$ which corresponds to the proportion of blocks updated per iteration $r$  closer to $1$ in terms of number of iterations. Contrarily, in terms of number of features processed $B=128$ has the best performance and $B=16$ has the worst performance. This shows that updating less features/coordinates per iterations can lead to faster convergence in terms of number of processed features.} \label{fig:rapsa_linear_hybrid}
\end{figure}


In Fig. \ref{subfig:rapsa_linear_constant_b}, we display the convergence of the excess mean square error $F(\bbx^t) - F(\bbx^*)$ in terms of number of features processed $\tilde{p}_t$. In doing so, we may clearly observe the advantages of updating fewer features/coordinates per iteration. Specifically, the different algorithms converge in a nearly identical manner, but RAPSA with $I<<B$ may be implemented without any complexity bottleneck in the dimension of the decision variable $p$ (also the dimension of the feature space).

%hybrid step-size RAPSA
We observe a comparable trend when we run RAPSA with a hybrid step-size scheme $\gamma^t= \min(\eps, \eps\tilde{T}_0/t)$ which is a constant $\eps=10^{-1.5}$ for the first $\tilde{T}_0=400$ iterations, after which it diminishes as $O(1/t)$. We again observe in Figure \ref{subfig:rapsa_linear_hybrid_a} that convergence is fastest in terms of excess mean square error versus iteration $t$ when all blocks are updated at each step. However, for this step-size selection, we see that updating fewer blocks per step is \emph{faster} in terms of number of features processed. 
%
%That is, to achieve the benchmark $F(\bbx^t)\leq 10^{6}$, we require $\tdp_t=1\times 10^3$, $\tdp_t=4.33\times 10^5$, $\tdp_t=1.99\times 10^5$, and $\tdp_t=1.15\times 10^5$ processed features, respectively, for the cases that the number of blocks are $B=16$, $B=32$, $B=64$, and $B=128$. 
%
This result shows that updating fewer coordinates per iteration yields convergence gains in terms of number of features processed. This advantage comes from the advantage of Gauss-Seidel style block selection schemes in block coordinate methods as compared with Jacobi schemes. In particular, it's well understood that for problems settings with specific conditioning, cyclic block updates are superior to parallel schemes, and one may respectively interpret RAPSA as compared to parallel SGD as executing variants of cyclic or parallel block selection schemes. We note that the magnitude of this gain is dependent on the condition number of the Hessian of the expected objective $F(\bbx)$.

%Consider one path over the dataset for the cases that $B=16$ and $B=32$. In $B=16$, given $\bbx^t$, we update all the $1024$ coordinates/features to update $\bbx^t$ and compute $\bbx^{t+1}$. On the other hand, for the case that $B=32$, we update $512$ features of $\bbx^t$ and get $\bbx^{t+1}$. Then we use the updated variable $\bbx^{t+1}$ to update the rest of coordinates and compute $\bbx^{t+2}$. This observation shows that $B=16$ acts as a Jacobi method, updating all coordinates of $\bbx$ in parallel, while $B>16$ has the structure of Gauss-Seidel method makes use of the updated information as it proceeds to update different coordinates. The superior behavior of Gauss-Seidel techniques as compared to Jacobi methods is well known, and underlies the performance gains in Fig. \ref{subfig:linear_b}.



 %%%%%%%%%
%%%   A   R   A   P   S   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%constant step-size Accelerated RAPSA
{\bf Results for Accelerated RAPSA} We now study the benefits of incorporating approximate second-order information about the objective $F(\bbx)$ into the algorithm in the form of ARAPSA (Algorithm \ref{algo_ARAPS}). We first run ARAPSA for the linear regression problem outlined above when using a constant step-size $\gamma^t=\gamma=10^{-2}$ with fixed mini-batch size $L=10$. Moreover, we again vary the number of blocks as  $B=16$, $B=32$, $B=64$, and $B=128$, corresponding to updating all, half, one-quarter, and one-eighth  of the elements of vector $\bbx$ per iteration, respectively. 
%\blue{We need a couple sentences about the different way we measure complexity for ARAPSA vs. RAPSA}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}\centering
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$]{
\includegraphics[width=0.48\linewidth,height=0.28\linewidth]
{figures/arapsa_linear_regression_empiricalrisk_constant_iter.eps}\label{subfig:arapsa_linear_constant_a}}
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.48\linewidth,height=0.28\linewidth]
{figures/arapsa_linear_regression_empiricalrisk_constant_features.eps}\label{subfig:arapsa_linear_constant_b}}
%
\caption{ARAPSA on a linear regression problem with signal dimension $p=1024$ for $N=10^3$ iterations with mini-batch size $L=10$ for different number of blocks $B=\{16,32,64,128\}$. We use constant step-size $\gamma^t= \gamma=10^{-1}$ using initialization $10^4 \times \bbone$. Convergence is comparable across the different cases in terms of number of iterations, but in terms of number of features processed $B=128$ has the best performance and $B=16$ (corresponding to parallelized oL-BFGS) converges slowest. We observe that using fewer coordinates per iterations leads to faster convergence in terms of number of processed elements of $\bbx$.} \label{fig:arapsa_linear_constant}
\end{figure}


 Fig. \ref{subfig:arapsa_linear_constant_a} displays the convergence path of ARAPSA's excess mean-square error $F(\bbx^t) - F(\bbx^*)$ versus the number of iterations $t$. We observe that parallelized oL-BFGS ($I=B$) converges fastest in terms of iteration index $t$. On the contrary, in Figure \ref{subfig:arapsa_linear_constant_b}, we may clearly observe that larger $B$, which corresponds to using \emph{fewer} elements of $\bbx$ per step, converges faster in terms of number of features processed. The Gauss-Seidel effect is more substantial for ARAPSA as compared with RAPSA due to the fact that the $\argmin$ of the instantaneous objective computed in block coordinate descent is better approximated by its second-order Taylor-expansion (ARAPSA, Algorithm \ref{algo_ARAPS}) as compared with its linearization (RAPSA, Algorithm \ref{algo_RAPSA}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}\centering
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$]{
\includegraphics[width=0.48\linewidth,,height=0.28\linewidth]
{figures/arapsa_linear_regression_empiricalrisk_hybrid_iter.eps}\label{subfig:arapsa_linear_hybrid_a}}
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.48\linewidth,height=0.28\linewidth]
{figures/arapsa_linear_regression_empiricalrisk_hybrid_features.eps}
\label{subfig:arapsa_linear_hybrid_b}}
%
\caption{ARAPSA on a linear regression problem with signal dimension $p=1024$ for $N=10^4$ iterations with mini-batch size $L=10$ for different number of blocks $B=\{16,32,64,128\}$. We use hybrid step-size $\gamma^t= \min(10^{-1.5},10^{-1.5} \tilde{T}_0/t)$ with annealing rate $\tilde{T}_0=400$. Convergence is comparable across the different cases in terms of number of iterations, but in terms of number of features processed $B=128$ has the best performance and $B=16$ has the worst performance. This shows that updating less features/coordinates per iterations leads to faster convergence in terms of number of processed features.} \label{fig:arapsa_linear_hybrid}
\end{figure}

%hybrid step-size Accelerated RAPSA
We now consider the performance of ARAPSA when a hybrid algorithm step-size is used, i.e. $\gamma^t= \min(10^{-1.5},10^{-1.5} \tilde{T}_0/t)$ with attenuation threshold $\tilde{T}_0=400$. The results of this numerical experiment are given in Figure \ref{fig:arapsa_linear_hybrid}. We observe that the performance gains of ARAPSA as compared to parallelized oL-BFGS apparent in the constant step-size scheme are more substantial in the hybrid setting. That is, in Figure \ref{subfig:arapsa_linear_hybrid_a} we again see that parallelized oL-BFGS is best in terms of iteration index $t$ -- to achieve the benchmark $F(\bbx^t) - F(\bbx^*)\leq 10^{-4}$, the algorithm requires $t=100$, $t=221$, $t=412$, and $t>1000$ iterations for $B=16$, $B=32$, $B=64$, and $B=128$, respectively. However, in terms of $\tilde{p}_t$, the number of elements of $\bbx$ processed, to reach the benchmark $F(\bbx^t) - F(\bbx^*)\leq 0.1$, we require $\tilde{p}_t > 1000$, $\tilde{p}_t=570$, $\tilde{p}_t=281$, and $\tilde{p}_t=203$, respectively, for $B=16$, $B=32$, $B=64$, and $B=128$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% C O M P A R I S O N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\bf Comparison of RAPSA and ARAPSA} 
%
We turn to numerically analyzing the performance of Accelerated RAPSA and RAPSA on the linear estimation problem for the case that parameter vectors $\bbx\in\reals^p$ are $p=500$ dimensional for $N=10^4$ iterations in the constant step-size case $\gamma=10^{-2}$. Both algorithms are initialized as $\bbx_0 = 10^3 \times \bbone$ with mini-batch size $L=10$, and ARAPSA uses the curvature memory level $\tau=10$. The number of processors is fixed again as $I=16$, and the number of blocks is $B=64$, meaning that $r=1/4$ of the elements of $\bbx$ are operated on at each iteration.  

The results of this numerical evaluation are given in Figure \ref{fig:rapsa_vs_arapsa_linear}. We plot the objective error sequence versus iteration $t$ in Figure \ref{subfig:rapsa_vs_arapsa_linear_a}. Observe that ARAPSA converges to within $10^{-4}$ of the optimum by $t=300$ iterations in terms of $F(\bbx^t) - F(\bbx^*)$, whereas RAPSA, while descending slowly, approaches within $10$ of the optimum by $t= 10^4$ iterations. The performance advantages of ARAPSA as compared to RAPSA are also apparent in Figure \ref{subfig:rapsa_vs_arapsa_linear_b}, which readjusts the results of Figure \ref{subfig:rapsa_vs_arapsa_linear_a} to be in terms of \emph{actual} elapsed time. We see that despite the higher complexity of ARAPSA per iteration, its empirical performance results in extremely fast convergence on linear estimation problems. That is, in about $3$ seconds, the algorithm converges to within $10^{-4}$ of the optimal estimator in terms of objective function evaluation.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}\centering
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$]{
\includegraphics[width=0.48\linewidth,,height=0.28\linewidth]
{figures/rapsa_vs_arapsa_iterations_linear.eps}\label{subfig:rapsa_vs_arapsa_linear_a}}
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. clock time (s)]{
\includegraphics[width=0.48\linewidth,,height=0.28\linewidth]
{figures/rapsa_vs_arapsa_clocktime_linear.eps}\label{subfig:rapsa_vs_arapsa_linear_b}}
%
\caption{A numerical comparison of RAPSA and ARAPSA on the linear estimation problem stated at the beginning of Section \ref{subsec:lmmse} for $N=10^4$ iterations with signal dimension $p=500$ with constant step-size $\gamma=10^{-2}$ when there are $I=16$ processors and $B=64$ blocks, meaning that one quarter of the elements of $\bbx$ are updated per iteration. Observe that the rate of convergence for ARAPSA is empirically orders of magnitude higher than RAPSA.} \label{fig:rapsa_vs_arapsa_linear}
\end{figure}



 %%%%%%%%%
%%%   A S Y N C H R O N O U S      R   A   P   S   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Results for Asynchronous RAPSA} 
%
We turn to studying the empirical performance of the asynchronous variant of RAPSA (Algorithm \ref{algo_asyn}) proposed in Section \ref{subsec:asynchronous}. The model we use for asynchronicity is modeled after a random delay phenomenon in physical communication systems in which each local server has a distinct clock which is not locked to the others. Each processor's clock begins at time $t_0^i=t_0$ for all processors $i=1,\dots,I$ and selects subsequent times as $t_{k} = t_{k-1} + w_k^i$, where $w_k^i \sim \ccalN(\mu,\sigma^2)$ is a normal random variable with mean $\mu$ and variance $\sigma^2$. The variance in this model effectively controls the amount of variability between the clocks of distinct processors. 

We run Asynchronous RAPSA for the linear estimation problem when the parameter vector $\bbx$ is $p=500$ dimensional for $N=10^3$ iterations with no mini-batching $L=1$ for both the case that the algorithm step-size is diminishing and constant step-size regimes for the case that the noise distribution perturbing the collected observations has variance $\sigma^2=10^{-2}$, and the observation matrix is as discussed at the outset of Section \ref{subsec:lmmse}. Further, the algorithm is initialized as $\bbx_0 = 10^3\bbone$. We run the algorithm for a few different instantiations of asynchronicity, that is, $w_k^i \sim \ccalN(\mu,\sigma^2)$ with $\mu = 1$ or $\mu = 2$, and $\sigma=.1$ or $\sigma = .3$.

The results of this numerical experiment are given in Figure \ref{fig:asyn_rapsa_linear} for both the constant and diminishing step-size schemes. We see that the performance of the asynchronous parallel scheme is comparable across different levels of variability among the local clocks of each processor. In particular, in Figure \ref{subfig:asyn_rapsa_linear_a} which corresponds to the case where the algorithm is run with constant step-size $\gamma=10^{-2}$, we observe comparable performance in terms of the objective function error sequence  $F(\bbx^t) - F(\bbx^*)$ with iteration $t$ -- across the varying levels of asynchrony we have  $F(\bbx^t) - F(\bbx^*)\leq 10$ by $t=10^3$. This trend may also be observed in the diminishing step-size scheme $\gamma^t=1/t$ which is given in Figure \ref{subfig:asyn_rapsa_linear_b}. That is, the distance to the optimal objective is nearly identical across differing levels of asynchronicity. In both cases, the synchronized algorithm performs better than its asynchronous counterpart.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering 
%
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$.]{
\includegraphics[width=0.45\linewidth,height=0.25\linewidth]
		{figures/rapsa_asynchronous_linear_constant.eps}\label{subfig:asyn_rapsa_linear_a}}
\subfigure[Excess Error $F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$.]{
\includegraphics[width=0.45\linewidth,height=0.25\linewidth]
                {figures/rapsa_asynchronous_linear_diminishing.eps}\label{subfig:asyn_rapsa_linear_b}}       
           %
\caption{Asynchronous RAPSA (Algorithm \ref{algo_asyn}) on the linear estimation problem in the constant ($\gamma=10^{4}$, left) and diminishing ($\gamma_t=10^6/(t + 250)$, right) step-size schemes with no mini-batching $L=1$ for a binary training subset of size $N=10^3$ with no regularization $\lambda=0$ when the algorithm is initialized as $\bbx_0 =10^3\times\bbone $. Varying the asynchronicity distribution has little effect, but we find that convergence behavior is slower than its synchronized counterpart, as expected.}\label{fig:asyn_rapsa_linear}
\end{figure}
%
%asynchronous RAPSA with constant step-size
%
%
%asynchronous RAPSA with diminishing step-size

 %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%MNIST  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Hand-Written Digit Recognition}\label{subsec:mnist}

We now make use of RAPSA for visual classification of written digits. To do so, let $\bbz\in\reals^p$ be a feature vector encoding pixel intensities (elements of the unit interval $[0,1]$ with smaller values being closer to black) of an image and let $y\in \{-1,1\}$ be an indicator variable of whether the image contains the digit $0$ or $8$, in which case the binary indicator is respectively $y=-1$ or $y=1$.
We model the task of learning a hand-written digit detector as a logistic regression problem, where one aims to train a classifier $\bbx \in \reals^p$ to determine the relationship between feature vectors $\bbz_n \in \reals^p$ and their associated labels $y_n \in \{-1,1\}$  for $n=1,\dots,N$. 
% 
The instantaneous function $f_n$ in \eqref{eq:empirical_min} for this setting is the $\lambda$-regularized negative log-likelihood of a generalized linear model of the odds ratio of whether the label is $y_n=1$ or $y_n=-1$. 
The empirical risk minimization associated with training set $\ccalT=\{(\bbz_n,y_n)\}_{n=1}^N$ is to find $\bbx^*$ as the maximum a posteriori estimate
% 
\begin{equation}\label{logistic_regression}
\bbx^* := \argmin_{\bbx\in\reals^p}  \frac{\lambda}{2}\|\bbx\|^2 + \frac{1}{N}\sum_{n=1}^N \log (1 + \exp({-y_n \bbx^T \bbz_n}))\; ,
\end{equation}
%
where the regularization term $({\lambda}{/2})\|\bbx\|^2$ encodes a prior belief on the joint distribution of $(\bbz, y)$ and helps to avoid overfitting. We use the MNIST dataset \citep{citeulike:599493}, in which feature vectors $\bbz_n \in \reals^p$ are $p=28^2=784$ pixel images whose values are recorded as intensities, or elements of the unit interval $[0,1]$. Considered here is the subset associated with digits $0$ and $8$, a training set $\ccalT=\{\bbz_n,y_n\}_{n=1}^N$ with $N=1.76\times 10^4$ sample points. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering 
%
\subfigure[Objective $F(\bbx^t)$ vs. iteration $t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
		{figures/rapsa_logistic_regression_objective_constant_iterations.eps}\label{subfig:rapsa_mnist_constant_a}}
\subfigure[Objective $F(\bbx^t)$ vs. feature $\tilde{p}_t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
                {figures/rapsa_logistic_regression_objective_constant_features.eps}\label{subfig:rapsa_mnist_constant_b}}
\subfigure[Test Set Accuracy vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.32\linewidth, height=0.2\linewidth]
                {figures/rapsa_logistic_regression_accuracy_constant_features.eps}\label{subfig:rapsa_mnist_constant_c}}                
           %
\caption{RAPSA on MNIST data with constant step-size $\gamma^t= \gamma=10^{-.5}$ with no mini-batching $L=1$. Algorithm performance is best in terms of number of iterations $t$ when all blocks are used per step (parallelized SGD), but in terms of number of features processed, the methods perform comparably. Thus RAPSA performs as well as SGD while breaking the complexity bottleneck in $p$, the dimension of decision variable $\bbx$.} \label{fig:rapsa_mnist_constant}
\end{figure}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering 
%
\subfigure[Objective $F(\bbx^t)$ vs. iteration $t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
		{figures/rapsa_logistic_regression_objective_hybrid_iterations.eps}\label{subfig:rapsa_mnist_hybrid_a}}
\subfigure[Objective $F(\bbx^t)$ vs. feature $\tilde{p}_t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
                {figures/rapsa_logistic_regression_objective_hybrid_features.eps}\label{subfig:rapsa_mnist_hybrid_b}}
\subfigure[Test Set Accuracy vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.32\linewidth, height=0.2\linewidth]
                {figures/rapsa_logistic_regression_accuracy_hybrid_features.eps}\label{subfig:rapsa_mnist_hybrid_c}}                
           %
\caption{RAPSA on MNIST data with hybrid step-size $\gamma^t= \min(10^{-3/4},10^{-3/4} \tilde{T}_0/t)$, with $\tilde{T}_0=300$ and no mini-batching $L=1$. As with the constant step-size selection, we observe that updating all blocks per iteration is best in terms of $t$, but in terms of elements of $\bbx$ updated, algorithm performance is nearly identical, meaning that no price is payed for breaking the complexity bottleneck in $p$.} \label{fig:rapsa_mnist_hybrid}
\end{figure}
%
 %%%%%%%%%
%%%    R   A   P   S   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Results for RAPSA} We run RAPSA on this training subset for the cases that $B=16$, $B=32$, $B=64$, and $B=128$, which are associated with updating $p$, $p/2$, $p/4$, and $p/8$ features per iteration. We consider the use of RAPSA with both constant and hybrid step-size selections. In Figure \ref{fig:rapsa_mnist_constant}, we display the results when we select a constant learning rate $\gamma^t=\gamma=10^{-.5}=0.316$. In Figure \ref{subfig:rapsa_mnist_constant_a} we plot the objective $F(\bbx^t)$ versus iteration $t$, and observe that algorithm performance improves with using more elements of $\bbx$ per iteration. That is, using all $p$ coordinates of $\bbx$ achieves superior convergence with respect to iteration $t$. 
%
However, as previously noted, iteration index $t$ is an unfair comparator for objective convergence since the four different setting process different number of features per iteration. In Figure \ref{subfig:rapsa_mnist_constant_b}, we instead consider $F(\bbx^t)$ versus the number of coordinates of $\bbx$, denoted as $\tilde{p}_t$, that algorithm performance is comparable across the different selections of $B$. This demonstrates that RAPSA breaks the computational bottleneck in $p$ while suffering no reduction in convergence speed with respect to $\tilde{p}_t$.

We consider further the classification accuracy on a test subset of size $\tilde{N}=5.88\times10^3$, the results of which are shown in Fig. \ref{subfig:rapsa_mnist_hybrid_c}. We see that the result for classification accuracy on a test set is consistent with the results for the convergence of the objective function value, and asymptotically reach approximately $98\%$ across the different instances of RAPSA.

In Figure \ref{fig:rapsa_mnist_hybrid} we show the result of running RAPSA for this logistic regression problem with hybrid step-size $\gamma^t= \min(10^{-3/4},10^{-3/4} \tilde{T}_0/t)$, with $\tilde{T}_0=300$ and no mini-batching $L=1$. In Fig. \ref{subfig:rapsa_mnist_hybrid_a}, which displays the objective $F(\bbx^t)$ versus iteration $t$, that using full stochastic gradients is better than only updating \emph{some} of the coordinates in terms of the number of iterations $t$. In particular, to reach the objective benchmark $F(\bbx^t) \leq 10^{-1}$, we have to run RAPSA $t=74$, $t=156$, and $t=217$, and $t=631$ iterations, for the cases that $B=16$, $B=32$, $B=64$, and $B=128$.
%
We illustrate  the objective $F(\bbx^t)$ vs. feature $\tilde{p}_t$ in Fig. \ref{subfig:rapsa_mnist_hybrid_b}. Here we recover the advantages of randomized incomplete parallel processing: updating fewer blocks per iteration yields comparable algorithm performance. %This demonstrates that RAPSA breaks the computational bottleneck in $p$ while suffering no reduction in convergence speed.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth,height = 0.45\linewidth]
%                {figures/mnist_accuracy_features2.eps}
%\caption{Test set accuracy vs. feature $\tilde{p}_t$.}
%\label{subfig:mnist3}
%\end{figure}

We additionally display the algorithm's achieved test-set accuracy on a test subset of size $\tilde{N}=5.88\times10^3$ in Fig. \ref{subfig:rapsa_mnist_hybrid_c} under the hybrid step-size regime. We again see that after a burn-in period, the classifier achieves the highly accurate asymptotic error rate of between $1-2\%$ across the different instantiations of RAPSA. We note that the test set accuracy achieved by the hybrid scheme is superior to the constant step-size setting.

%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{figure}[ht]
% \centering
% \subfigure[Empirical risk $F(\bbx^t) - F(\bbx^*)$ vs. iteration $\tilde{p}_t$]{
%  \includegraphics[width=0.48\linewidth,height=0.28\linewidth]{figures/rapsa_vs_arapsa_I=49_empiricalrisk.eps}
%   \label{subfig:rapsa_v_arapsa1}
%   }
% \subfigure[Classification accuracy vs. iteration $\tilde{p}_t$]{
%  \includegraphics[width=0.48\linewidth,height=0.28\linewidth]{figures/rapsa_vs_arapsa_I=49_accuracy.eps}
%   \label{subfig:rapsa_v_arapsa2}
%   }
% \caption{RAPSA and ARAPSA algorithms on MNIST data with mini-batch size $L=10$, the level of curvature information set to $\tau=10$, and constant step-size $\gamma=10^{-1}$. ARAPSA successfully accelerates the convergence of RAPSA, and achieves higher accuracy per features processed $\tilde{p}_t$.} \label{fig:rapsa_v_arapsa}
%\end{figure}


 %%%%%%%%%
%%%   A   R   A   P   S   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Results for Accelerated RAPSA} We now run Accelerated RAPSA (Algorithm \ref{algo_ARAPS}) as stated in Section \ref{sec:arapsa} for this problem setting for the entire MNIST binary training subset associated with digits $0$ and $8$, with mini-batch size $L=10$ and the level of curvature information set as  $\tau=10$. We further select regularizer $\lambda=1/\sqrt{N}=7.5\times 10^{-3}$, and consider both constant and hybrid step-size regimes. As before, we study the advantages of incomplete randomized parallel processing by varying the number of blocks $B\in \{16, 32, 64,128\}$ on an architecture with a fixed number $|\ccalI_t|=I=16$ of processors. This setup is associated with using all $p$ entries of vector $\bbx$ at each iteration as compared with $1/2$, $1/4$, and $1/8$ of its entries.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering 
%
\subfigure[Objective $F(\bbx^t)$ vs. iteration $t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
		{figures/arapsa_logistic_regression_objective_constant_iterations.eps}\label{subfig:arapsa_mnist_constant_a}}
\subfigure[Objective $F(\bbx^t)$ vs. feature $\tilde{p}_t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
                {figures/arapsa_logistic_regression_objective_constant_features.eps}\label{subfig:arapsa_mnist_constant_b}}
\subfigure[Test Set Accuracy vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.32\linewidth, height=0.2\linewidth]
                {figures/arapsa_logistic_regression_accuracy_constant_features.eps}\label{subfig:arapsa_mnist_constant_c}}                
           %
\caption{ARAPSA on MNIST data with constant step-size $\gamma^t= \gamma=10^{-2}$ and mini-batch size $L=10$, curvature memory $\tau=10$, and regularizer $\lambda=7.5\times10^{-3}$. Algorithm performance is comparable across different numbers of decision variable coordinates updated per iteration $t$, but in terms of number of features processed, ARAPSA performance best when using the least information per update.}\label{fig:arapsa_mnist_constant}
\end{figure}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering 
%
\subfigure[Objective $F(\bbx^t)$ vs. iteration $t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
		{figures/arapsa_logistic_regression_objective_hybrid_iterations.eps}\label{subfig:arapsa_mnist_hybrid_a}}
\subfigure[Objective $F(\bbx^t)$ vs. feature $\tilde{p}_t$.]{
\includegraphics[width=0.32\linewidth,height=0.2\linewidth]
                {figures/arapsa_logistic_regression_objective_hybrid_features.eps}\label{subfig:arapsa_mnist_hybrid_b}}
\subfigure[Test Set Accuracy vs. feature $\tilde{p}_t$]{
\includegraphics[width=0.32\linewidth, height=0.2\linewidth]
                {figures/arapsa_logistic_regression_accuracy_hybrid_features.eps}\label{subfig:arapsa_mnist_hybrid_c}}                
           %
\caption{ARAPSA on MNIST data with hybrid step-size $\gamma^t= \min(10^{-1},10^{-1} \tilde{T}_0/t)$, with $\tilde{T}_0=500$, mini-batch size $L=10$, curvature memory $\tau=10$, and regularizer $\lambda=7.5\times10^{-3}$. Algorithm performance is comparable across different numbers of decision variable coordinates updated per iteration $t$, but in terms of number of features processed, RAPSA performance best when using the least information per update.}\label{fig:arapsa_mnist_hybrid}
\end{figure}
%

Figures \ref{fig:arapsa_mnist_constant} the results of this algorithm run when a constant step-size $\gamma=10^{-2}$ is used. Observe in Figure \ref{subfig:arapsa_mnist_constant_a} that the algorithm achieves convergence across the differing numbers of blocks $B$ in terms of iteration $t$, with faster learning rates achieved with smaller $B$. In particular, to reach the benchmark $F(\bbx^t) \leq 10^{-1}$, we require $t=145$, $t=311$, and $t=701$ iterations for $B=16$, $B=32$, and $B=64$, respectively, whereas the case $B=128$ does not achieve this benchmark by $t=10^3$. This trend is inverted, however, in  Figure \ref{subfig:arapsa_mnist_constant_b}, which displays the objective $F(\bbx^t)$ with $\tilde{p}_t$ the number of coordinates of $\bbx$ on which the algorithm operates per step. Observe that using \emph{fewer} entries of $\bbx$ per iteration is better in terms of number of features processed $\tilde{p}_t$. Furthermore, ARAPSA achieves comparable accuracy on a test set of images, approximately near $98\%$ across different selections of $B$, as is displayed in Figure \ref{subfig:arapsa_mnist_constant_c}.


%for hybrid step-size
We now run Accelerated RAPSA when the learning rate is hand-tuned to optimize performance via a hybrid scheme $\gamma^t= \min(10^{-1},10^{-1} \tilde{T}_0/t)$, with attenuation threshold $\tilde{T}_0=500$. The results of this experiment are given in Figure \ref{fig:arapsa_mnist_hybrid}. In particular, in Figure \ref{subfig:arapsa_mnist_hybrid_a} we plot the objective $F(\bbx^t)$ with iteration $t$ when the number of blocks $B$ is varied. We see that parallelized oL-BFGS ($I=B$ so that $r=1$) performs best in terms of $t$: to achieve the threshold condition $F(\bbx^t) \leq 10^{-1}$, we require $t=278$, $t=522$ iterations for $B=16$ and $B=32$, respectively, whereas the cases $B=64$ and $B=128$ do not achieve this benchmark by $t=10^3$. However, the instance of ARAPSA with the fastest and most accurate convergence uses the \emph{least} coordinates of $\bbx$ when we compare the objective with $\tilde{p}_t$, as may be observed in Figure \ref{subfig:arapsa_mnist_hybrid_b}.  This trend is corroborated in Figure \ref{subfig:arapsa_mnist_hybrid_c}, where we observe that ARAPSA with $B=128$ achieves $99\%$ test-set accuracy the fastest, followed by $B=64$, $B=32$, and $B=16$.
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% C O M P A R I S O N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Comparison of RAPSA and ARAPSA} 
We now compare the performance of RAPSA and its accelerated variant on the MNIST digit recognition problem for a binary subset of the training data consisting of $N=10^5$ samples. We run both algorithms on an $I=16$ processor simulated architecture with $B=64$ blocks, such that $r=1/4$ of the elements of $\bbx$ are operated upon at each step. We consider the constant algorithm step-size scheme $\gamma=10^{-2}$ with mini-batch size $L=10$. 

The results of this online training procedure are given in \eqref{fig:rapsa_vs_arapsa_logistic}, where we plot the objective optimality gap $F(\bbx^t) - F(\bbx^*)$ versus the number of feature vectors processed $tL$ (Figure \ref{subfig:rapsa_vs_arapsa_logistic_a}) and actual elapsed time (Figure \ref{subfig:rapsa_vs_arapsa_logistic_b}). We see ARAPSA achieves superior convergence behavior with respect to RAPSA in terms of number of feature vectors processed: to achieve the benchmark $F(\bbx^t) - F(\bbx^*)\leq 10^{-1}$, ARAPSA requires fewer than $tL=200$ feature vectors, whereas RAPSA requires $tL=4\times10^4 $ feature vectors. This relationship is corroborated in Figure \ref{subfig:rapsa_vs_arapsa_logistic_b}, where we see that within a couple seconds ARAPSA converges to within $10^{-1}$, whereas after $\emph{five}$ times as long, RAPSA does not achieve this benchmark.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}\centering
%
\subfigure[$F(\bbx^t) - F(\bbx^*)$ vs. iteration $t$]{
\includegraphics[width=0.48\linewidth,,height=0.28\linewidth]
{figures/rapsa_vs_arapsa_iterations_logistic.eps}\label{subfig:rapsa_vs_arapsa_logistic_a}}
%
\subfigure[$F(\bbx^t) - F(\bbx^*)$ vs. clock time (s)]{
\includegraphics[width=0.48\linewidth,,height=0.28\linewidth]
{figures/rapsa_vs_arapsa_clocktime_logistic2.eps}\label{subfig:rapsa_vs_arapsa_logistic_b}}
%
\caption{A comparison of RAPSA and ARAPSA on the MNIST digit recognition problem for a binary training subset of size $N=10^3$ with mini-batch size $L=10$ in the constant step-size scheme $\gamma=10^{-2}$. The objective optimality gap $F(\bbx^t) - F(\bbx^*)$ is shown with respect to the number of feature vectors processed $tL$ (left) and actual elapsed time (right). While the performance difference between RAPSA and ARAPSA is not as large as in the linear estimation problem, we still observe that ARAPSA substantially accelerates the convergence of RAPSA for a standard machine learning problem.} \label{fig:rapsa_vs_arapsa_logistic}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% A S Y N C H R O N O U S     R A P S A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\bf Results for Asynchronous RAPSA} 
%
We now evaluate the empirical performance of the asynchronous variant of RAPSA (Algorithm \ref{algo_asyn}) proposed in Section \ref{subsec:asynchronous} on the logistic regression formulation of the MNIST digit recognition problem. The model we use for asynchronicity is the one outlined in Section \ref{subsec:lmmse}, that is, each local processor has a distinct local clock which is not required coincide with others, begins at time $t_0^i=t_0$ for all processors $i=1,\dots,I$, and then selects subsequent times as $t_{k} = t_{k-1} + w_k^i$. Here $w_k^i \sim \ccalN(\mu,\sigma^2)$ is a normal random variable with mean $\mu$ and variance $\sigma^2$ which controls the amount of variability between the clocks of distinct processors. We run the algorithm with no regularization $\lambda=0$ or mini-batching $L=1$ and initialization  $\bbx_0 =\bbone $.

The results of this numerical setup are given in Figure \ref{fig:asyn_rapsa_mnist}. We consider the expected risk $F(\bbx^t)$ in both both the constant ($\gamma=10^{-2}$, Figure \ref{subfig:asyn_rapsa_mnist_a}) and diminishing ($\gamma^t=1/t$, Figure \ref{subfig:asyn_rapsa_mnist_b}) algorithm step-size schemes. We see that the level of asynchronicity does not significantly impact the performance in either scheme, and that the convergence guarantees established in Theorem \ref{RAPSA_convg_thm_asyn} hold true in practice. We again observe that the version of RAPSA with synchronized computations converges at a faster rate than Asynchronous RAPSA.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering 
%
\subfigure[Objective $F(\bbx^t)$ vs. iteration $t$.]{
\includegraphics[width=0.45\linewidth,height=0.25\linewidth]
		{figures/rapsa_asynchronous_logistic_constant.eps}\label{subfig:asyn_rapsa_mnist_a}}
\subfigure[Objective $F(\bbx^t)$ vs. iteration $t$.]{
\includegraphics[width=0.45\linewidth,height=0.25\linewidth]
                {figures/rapsa_asynchronous_logistic_diminishing.eps}\label{subfig:asyn_rapsa_mnist_b}}       
           %
\caption{Asynchronous RAPSA on MNIST data in the constant ($\gamma=10^{-2}$, left) and diminishing ($\gamma^t=1/t$, right) step-size schemes with no mini-batching $L=1$ for a binary training subset of size $N=10^3$ with no regularization $\lambda=0$ when the algorithm is initialized as $\bbx_0 =\bbone $. The variability in local processor clocks does not significantly impact performance in both the diminishing and constant step-size settings; however, the synchronous algorithm converges at a faster rate.}\label{fig:asyn_rapsa_mnist}
\end{figure}
%
 
